A Logical Study of Some Common Principles of Inductive Definition and its Implications for Knowledge Representation

The definition is a common form of human expert knowledge, a building block of formal science and mathematics, a foundation for database theory and is supported in various forms in many knowledge representation and formal specification languages and systems. This paper is a formal study of some of the most common forms of inductive definitions found in scientific text: monotone inductive definition, definition by induction over a well-founded order and iterated inductive definitions. We define a logic of definitions offering a uniform formal syntax to express definitions of the different sorts, and we define its semantics by a faithful formalization of the induction process. Several fundamental properties of definition by induction emerge: the non-determinism of the induction process, the confluence of induction processes, the role of the induction order and its relation to the inductive rules, how the induction order constrains the induction process and, ultimately, that the induction order is irrelevant: the defined set does not depend on the induction order. We propose an inductive construction capable of constructing the defined set without using the induction order. We investigate borderline definitions of the sort that appears in definitional paradoxes.

==> idp-latex/common-citations.tex <==
\usepackage{etoolbox}

\newcommand\setcitation[2]{%
  \csdef{mycommoncitation#1}{#2}}
\newcommand\getcitation[1]{%
  \csuse{mycommoncitation#1}}

\setcitation{IDP}{WarrenBook/DeCatBBD14}
\setcitation{idp}{WarrenBook/DeCatBBD14}
\setcitation{fodot}{tocl/DeneckerT08}
\setcitation{CP}{Apt03}
\setcitation{cp}{Apt03}
\setcitation{EZCSP}{lpnmr/Balduccini11}
\setcitation{KR}{Baral:2003}
\setcitation{ASPComp2}{lpnmr/DeneckerVBGT09}
\setcitation{ASPComp3}{journals/tplp/CalimeriIR14}
\setcitation{ASPComp4}{conf/lpnmr/AlvianoCCDDIKKOPPRRSSSWX13}
\setcitation{CPSupport}{ictai/DeCat13}
\setcitation{CPsupport}{ictai/DeCat13}
\setcitation{functionDetection}{iclp/DeCatB13}
\setcitation{fodot2asp}{DeneckerLTV12} %TODO replace by journal publication if one is publishedr
\setcitation{Tarskian}{DeneckerLTV12} %Same as the one above 
\setcitation{Inca}{iclp/DrescherW12}
\setcitation{csp2asp}{ijcai/DrescherW11}
\setcitation{DPLLT}{cav/GanzingerHNOT04}
\setcitation{AspInPractice}{synthesis/2012Gebser}
\setcitation{clasp}{ai/GebserKS12}
\setcitation{oclingo}{kr/GebserGKOSS12}
\setcitation{gringo}{lpnmr/GebserST07}
\setcitation{cmodels}{aaai/GiunchigliaLM04}
\setcitation{inputster}{tplp/Jansen13}
\setcitation{DLV}{tocl/LeonePFEGPS06}
\setcitation{LearningPaper}{TPLP/BruynoogheBBDDJLRDV} %TODO replace by published version
\setcitation{clog}{iclp/BogaertsVDV14} %TODO replace by journal publication if one is published
\setcitation{foc}{iclp/BogaertsVDV14}
\setcitation{FOC}{iclp/BogaertsVDV14}
\setcitation{inferenceClog}{ecai/BogaertsVDV14}
\setcitation{examplesClog}{nmr/BogaertsVDV14b} %TODO replace by better publication if possible
\setcitation{AFT}{DeneckerBV12}
\setcitation{KBS}{iclp/DeneckerV08}
\setcitation{KBS-invitedtalk}{jelia/Denecker16}
\setcitation{KBPE}{inap/DePooterWD11}
\setcitation{lazyGrounding}{jair/CatDBS15} 
\setcitation{lazygrounding}{jair/CatDBS15} 
\setcitation{ASP}{marek99stable}
\setcitation{satid}{sat/MarienWDB08}
\setcitation{lazyclausegeneration}{constraints/OhrimenkoSC09}
\setcitation{FP}{ACMCS/Hudak89}
\setcitation{GroundingWithBounds}{jair/WittocxMD10}
\setcitation{SAT}{faia/SilvaLM09}
\setcitation{LTC}{iclp/Bogaerts14}
\setcitation{SPSAT}{ictai/DevriendtBMDD12}
\setcitation{BreakID}{sat/DevriendtBBD16}
\setcitation{breakid}{sat/DevriendtBBD16}
\setcitation{LCG}{stuckeyLCG}
\setcitation{MiniZinc}{conf/cp/NethercoteSBBDT07}
\setcitation{minizinc}{conf/cp/NethercoteSBBDT07}
\setcitation{amadini}{cpaior/AmadiniGM13}
\setcitation{bootstrapping}{ngc/BogaertsJDJBD16}
\setcitation{Bootstrapping}{ngc/BogaertsJDJBD16}
\setcitation{GroundedFixpoints}{ai/BogaertsVD15}
\setcitation{PartialGroundedFixpoints}{ijcai/BogaertsVD15}
\setcitation{LogicBlox}{datalog/GreenAK12}
\setcitation{proB}{journals/sttt/LeuschelB08}
\setcitation{NaturalInductions}{KR/DeneckerV14} %TODO replace by journal publication if one is published
\setcitation{LP}{jacm/EmdenK76}
\setcitation{SMT}{faia/BarrettSST09}
\setcitation{AF}{ai/Dung95}
\setcitation{ADF}{kr/BrewkaW10}
\setcitation{af}{ai/Dung95}
\setcitation{adf}{kr/BrewkaW10}
\setcitation{ADFRevisited}{ijcai/BrewkaSEWW13}
\setcitation{adfrevisited}{ijcai/BrewkaSEWW13}
\setcitation{DefaultLogic}{ai/Reiter80}
\setcitation{DL}{ai/Reiter80}
\setcitation{AEL}{mo85}
\setcitation{minisat}{sat/EenS03}
\setcitation{completion}{adbt/Clark78}
\setcitation{wasp}{lpnmr/AlvianoDFLR13}
\setcitation{minisatid}{ictai/DeCat13}
\setcitation{lcg}{stuckeyLCG}
\setcitation{CEGAR}{jacm/ClarkeGJLV03}
\setcitation{cegar}{jacm/ClarkeGJLV03}
\setcitation{CuttingPlane}{or/DantzigFJ54}
\setcitation{kodkod}{tacas/TorlakJ07}
\setcitation{cdcl}{Marques-SilvaS99}
\setcitation{CDCL}{Marques-SilvaS99}
\setcitation{relevance}{ijcai/JansenBDJD16}
\setcitation{relevance-implementation}{aspocp/JansenBDJD16}
\setcitation{WFS}{GelderRS91}
\setcitation{wfs}{GelderRS91}
\setcitation{UnfoundedSet}{GelderRS91}
\setcitation{stablesemantics}{iclp/GelfondL88}
\setcitation{StableSemantics}{iclp/GelfondL88}
\setcitation{shatter}{Shatter}
\setcitation{sbass}{drtiwa11a}
\setcitation{lparsemanual}{url:lparse_manual}
\setcitation{AIC}{ppdp/FlescaGZ04}
\setcitation{templates}{tplp/DassevilleHJD15}
\setcitation{templates2}{iclp/DassevilleHBJD16}
\setcitation{sat-to-sat}{aaai/JanhunenTT16}
\setcitation{sat-to-sat-qbf}{bnp/BogaertsJT16}
\setcitation{sat-to-sat-QBF}{bnp/BogaertsJT16}
\setcitation{sat-to-sat-SO}{kr/BogaertsJT16}
\setcitation{XSB}{SwiW12}
\setcitation{KCmap}{jair/DarwicheM02}
\setcitation{TLA}{DBLP:books/aw/Lamport2002}
\setcitation{EventB}{BookAbrial2010}
\setcitation{MX}{MitchellTHM06}
\setcitation{MIP}{Sierksma96}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
\setcitation{}{}
  
 %Command for in case you want multiple citations in one, e.g., \cite{\refto{fodot},\refto{idp}}
 %Warning: no safety checks
\newcommand\refto[1]{%
      \getcitation{#1}}
      
 %usage: \mycite{key}, e.g., \mycite{fodot} results in \cite{tocl/DeneckerT08}
\newcommand\mycite[1]{%
      \ifcsname mycommoncitation#1\endcsname%
   \cite{\getcitation{#1}}%
  \else%
    \cite{#1}%
  \fi%
}	
  
   %usage: \mycite{key}, e.g., \mycite{fodot} results in \cite{tocl/DeneckerT08}
\newcommand\mycitet[1]{%
      \ifcsname mycommoncitation#1\endcsname%
   \citet{\getcitation{#1}}%
  \else%
    \citet{#1}
  \fi%
}	
  


==> idp-latex/idp-latex-no-theorem.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex-no-theorem}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}




%The following are directives for LaTeX editors that collect ``included files'' to autocomplete macros etcetera
\ignore{
\include{includes-no-theorems}
\include{common-citations}
}

==> idp-latex/idp-latex.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}
\subimport{idp-latex/}{theorems}







%The following are directives for LaTeX editors that collect ``included files'' to autocomplete macros etcetera
\ignore{
\include{includes-no-theorems}
\include{common-citations}
\include{theorems}
}

==> idp-latex/idp-listings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             Stuff for writing IDP source code with coloring              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\usepackage[final]{listings}

	\lstdefinelanguage{idp}{
		morekeywords=[1]{query(}, %to ignore procedure calls to query
		morekeywords=[2]{namespace,vocabulary,theory,structure,procedure,term,set,formula, spec, specification,query},
		morekeywords=[3]{include,using,type,isa,contains,partial,extern,LFD,GFD,constructed,from,constraint,pred,supertype,of,subtype,define},
		morekeywords=[4]{int,float,char,string,nat},
		morekeywords=[5]{if,then,else,for,end},
		morecomment=[s]{/*}{*/},	
		morecomment=[l]{//}
	}
	\lstset{
		language=idp,
		tabsize=3,
		basicstyle=\small,
		frame=none,
		frame=single,
		showstringspaces=false,
		breaklines = true,
		alsoletter=(,
		commentstyle=\commentstyle,
		keywordstyle=[1],
		keywordstyle=[2]\color{BrickRed}\bfseries,
		keywordstyle=[3]\color{OliveGreen}\bfseries,
		keywordstyle=[4]\color{Blue}\bfseries,
		keywordstyle=[5]\color{Violet}\bfseries,
		literate={~} {$\sim$}{1}
	}
	\newcommand{\code}[1]{\texttt{#1}}


==> idp-latex/includes-no-theorems.tex <==
\usepackage{ifthen}
\usepackage{url}
% \usepackage{cite} DOES NOT WORK WITH ALL STYLES
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{import}
\subimport{packages/}{xparse}
\usepackage{amsmath}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{xspace}
\usepackage{datatool}
\usepackage{glossaries}

%ensured math mode with correct spacing
\providecommand\m[1]{\ensuremath{#1}\xspace}
\renewcommand{\m}[1]{\ensuremath{#1}\xspace}
\newcommand{\trval}[1]{\m{\mathbf{#1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%         LOGICAL STUFF: Operators, theories, ....         %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%NOTE: arrows are not surrounded by the \m command. THe reason is that they are math operators that have
% other spacing 
% For instance: L\to L has spacing between L and \to and betwee \to and L, while L{\to}L does not. 

%% Logic
% lor, land, lnot are standard. Extensions:
	\newcommand{\limplies}{\Rightarrow}
	\newcommand{\limpl}{\limplies}
	\newcommand{\lequiv}{\Leftrightarrow}
	\newcommand{\limpliedby}{\Leftarrow}
	\newcommand{\limplied}{\limpliedby}
	\newcommand{\lrule}{\leftarrow}
	\newcommand{\cause}{\stackrel{c}{\lrule}}
	\newcommand{\rul}{\leftarrow}
	\newcommand{\ltrue}{\trval{t}}
	\newcommand{\lfalse}{\trval{f}}
	\newcommand{\lunkn}{\trval{u}}
	\newcommand{\lincon}{\trval{i}}
%related
	\newcommand{\bigand}{\bigwedge}
	\newcommand{\bigor}{\bigvee}
	\newcommand{\true}{\m{\top}}
	\newcommand{\false}{\m{\bot}}
% Marc zijn versies
	\newcommand{\Lra}{\Leftrightarrow}
	\newcommand{\lra}{\leftrightarrow}
	\newcommand{\Ra}{\Rightarrow}
	\newcommand{\La}{\Leftarrow}
	\newcommand{\ra}{\rightarrow}
	\newcommand{\la}{\leftarrow}
	\newcommand{\mim}{\limplies}
	\newcommand{\equi}{\lequiv}
	\newcommand{\Tr}{\ltrue}
	\newcommand{\Fa}{\lfalse}
	\newcommand{\Un}{\lunkn}
	\newcommand{\In}{\lincon}
	
%Vocabularies, structures, theories
	\newcommand{\voc}{\m{\Sigma}}
	\newcommand{\invoc}{\m{\sigma_{in}}}
	\newcommand{\outvoc}{\m{\sigma_{out}}}
	\newcommand{\struct}{\m{I}}
	\newcommand{\structx}{\m{I}}
	\newcommand{\I}{\m{\mathcal{I}}}
	\newcommand{\Iin}{\m{\I_{in}}}
	\newcommand{\J}{\m{\mathcal{J}}}
	\newcommand{\instruct}{\m{I_{in}}}
	\newcommand{\outstruct}{\m{I_{out}}}
	\newcommand{\theory}{\m{\mathcal{T}}}

%More caligraphic characters
	\newcommand{\PP}{\m{\mathcal{P}}}
	\newcommand{\LL}{\m{\mathcal{L}}}
	\newcommand{\WW}{\m{\mathcal{W}}}
	\newcommand{\BB}{\m{\mathcal{B}}}


%Often used abbreviations for definitions, formulas,...
	\newcommand{\D}{\m{\Delta}}
	\newcommand{\f}{\m{\varphi}}
	\newcommand{\atom}{\m{a}}
	\newcommand{\lit}{\m{l}}
	\newcommand{\rules}{\m{R}}
	\newcommand{\set}{\m{S}}
	\NewDocumentCommand\inter{g+g}{%
	  \IfNoValueTF{#1}
	    {\struct}
	    {\m{#1^{#2}}}}
	\newcommand{\partinter}{\m{J}}
	\newcommand{\model}{\m{M}}
	\newcommand{\fone}{\m{\varphi}}
	\newcommand{\ftwo}{\m{\psi}}

%properties of definitions
	\newcommand{\defined}[1]{\ensuremath{\mbox{\it Def}({#1})}\xspace}
	\newcommand{\open}[1]{\ensuremath{\mbox{\it Open}({#1})}\xspace}
	\newcommand{\pars}[1]{\ensuremath{\mbox{\it Par}({#1})}\xspace}
	\newcommand{\just}{\m{just}}

% Inferences
	\newcommand{\mx}[3]{\m{<#1, #2, #3>}}

%Vectors
	\newcommand{\xxx}{\m{\overline{x}}}
	\newcommand{\XXX}{\m{\overline{X}}}
	\newcommand{\yyy}{\m{\overline{y}}}
	\newcommand{\zzz}{\m{\overline{z}}}
	\newcommand{\ddd}{\m{\overline{d}}}
	\newcommand{\eee}{\m{\overline{e}}}
	\newcommand{\ccc}{\m{\overline{c}}}
	\newcommand{\bracketddd}{\m{\big(\overline{d}\big)}}
	\newcommand{\bddd}{\m{\big(\overline{d}\big)}}
	\newcommand{\DDD}{\m{\overline{D}}}
	\newcommand{\vvv}{\m{\overline{v}}}
	\newcommand{\ttt}{\m{\overline{t}}}
	\newcommand{\aaa}{\m{\overline{a}}}
	\newcommand{\bbb}{\m{\overline{b}}}
 	\providecommand{\lll}{\m{\overline{l}}}%sometimes, already exists
 	\renewcommand{\lll}{\m{\overline{l}}}
	\newcommand{\TTT}{\m{\overline{T}}}

%Set operations
	\newcommand{\elim}{\m{\backslash}}
	
%Rewrite rules
	\newcommand{\transformarrow}{\pmb{\pmb\rightarrowtail}}
	\newcommand{\rewrite}[2]{\m{#1  \ \transformarrow\    #2 }}

% Common Base types
	\newcommand{\bool}{\m{\mathbb{B}}}
	\newcommand{\Bool}{\bool}
	\newcommand{\nat}{\m{\mathbb{N}}}
	\newcommand{\Nat}{\nat}
	\renewcommand{\int}{\m{\mathbb{Z}}}
	\newcommand{\real}{\m{\mathbb{R}}}
	\newcommand{\rat}{\m{\mathbb{Q}}}

% Precision order
	\newcommand{\leqp}{\m{\leq_p}}
	\newcommand{\geqp}{\m{\geq_p}}
	\newcommand{\leqk}{\m{\leq_k}}
	\newcommand{\geqk}{\m{\geq_k}}
	\newcommand{\leqt}{\m{\leq_t}}
	\newcommand{\geqt}{\m{\geq_t}}
	
%Lattice operators
	\DeclareMathOperator\glb{glb}
	\DeclareMathOperator\lub{lub}
	\DeclareMathOperator\lfp{lfp}
	\DeclareMathOperator\gfp{gfp}


%valuations
	\newcommand{\val}{\m{\nu}}
	\newcommand{\superval}{\m{sv}}
	\newcommand{\kleeneval}{\m{Kl}}



%other
	\newcommand{\typed}[2]{\m{#1\in #2:}}
	\newcommand{\hasmodel}{\mid\!\equiv}
	\NewDocumentCommand\subs{g+g}{%
	  \IfNoValueTF{#1}
	    {\m{/}}
	    {\m{#1/ #2}}}
	\newcommand{\substitute}[2]{\subs{#1}{#2}}	
	\newcommand{\func}[1]{\m{f(#1)}}
	\newcommand{\setof}[1]{\m{\left \{ #1 \right \}}}
	\newcommand{\tuple}[1]{\m{\left \langle #1 \right \rangle }}
	\newcommand{\til}{\m{\sim}}
	\newcommand\eqdef{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%                    Logics and systems                    %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%General command to ensure correct spacing and text mode
	\newcommand{\logicname}[1]{\textsc{#1}\xspace}

%Systems
	\newcommand{\idp}{\logicname{IDP}}
	\newcommand{\xsb}{\logicname{XSB}}
	\newcommand{\idptwo}{\logicname{IDP$^2$}}
	\newcommand{\idpthree}{\logicname{IDP3}}
	\newcommand{\idpfour}{\logicname{IDP4}}
	\newcommand{\idpdraw}{\logicname{ID$^{P}_{Draw}$}}
	\newcommand{\idpide}{\logicname{ID$^{P}_{E}$}}
	\newcommand{\minisat}{\logicname{MiniSAT}}
	\newcommand{\minisatid}{\logicname{MiniSAT(ID)}}
	\newcommand{\gidl}{\logicname{GidL}}
	\newcommand{\sts}{\logicname{SAT-to-SAT}}
	\newcommand{\breakid}{\logicname{BreakID}}
	\newcommand{\glucose}{\logicname{Glucose}}
	\newcommand{\shatter}{\logicname{Shatter}}
	\newcommand{\saucy}{\logicname{Saucy}}
	\newcommand{\sbass}{\logicname{sbass}}
	\newcommand{\nauty}{\logicname{nauty}}
	\newcommand{\bliss}{\logicname{bliss}}
	\newcommand{\gringo}{\logicname{gringo}}
	\newcommand{\lparse}{\logicname{Lparse}}
	\newcommand{\smodels}{\logicname{Smodels}}
	

	
%logics
	\newcommand{\fodotidp}{\logicname{FO(\ensuremath{\cdot})\ensuremath{^{\mathtt{IDP}}}}}
	\newcommand{\foidp}{\fodotidp}
	\newcommand{\fodot}{\logicname{FO(\ensuremath{\cdot})}}
	\newcommand{\pcdot}{\logicname{PC(\ensuremath{\cdot})}}
	\newcommand{\foid}{\logicname{FO(ID)}}
	\newcommand{\foidaggpf}{\logicname{FO(ID,\allowbreak Agg,\allowbreak PF)}}
	\newcommand{\foidaggpft}{\logicname{FO(ID,\allowbreak Agg,\allowbreak PF,\allowbreak T)}}
	\newcommand{\foidplus}{\logicname{C-Log}} %DEPRECATED
	\newcommand{\clog}{\logicname{C-Log}}
	\newcommand{\foclog}{\logicname{FO(C)}}
	\newcommand{\hoid}{\logicname{HO(ID)}}
	\newcommand{\hopfid}{\logicname{HO(PF,ID)}}
	\newcommand{\fo}{\FO}
	\newcommand{\esoid}{\logicname{\ensuremath{\exists}SO(ID)}}
	\newcommand{\cpl}{\logicname{CP}-logic\xspace}
	\newcommand{\aspcore}{\text{\sc ASP-Core-2}\xspace}

%acronyms. USAGE: \ouracronym{CommandName}{A}{Acronym} creates a command \CommandName such that:
% * The first time you write it (probably the moment you define it), it reads Acronym (A)
% * All later times you use it, it simply says A.
% NOTE: to reset the counter, use \glsreset{<label>}
\newcommand{\ouracronym}[3]{%
	\newacronym{#1}{#2}{#3}
	\expandafter\newcommand\csname #1\endcsname{\gls{#1}\xspace}%
}
	\ouracronym{FO}{FO}{first-order logic}
	\ouracronym{PC}{PC}{propositional calculus}
	\ouracronym{MX}{MX}{Model Expansion}
	\ouracronym{MO}{MO}{Model Optimization}
	\ouracronym{ASP}{ASP}{Answer Set Programming}
	\ouracronym{TP}{TP}{Theorem Proving}
	\ouracronym{LP}{LP}{Logic Programming}
	\ouracronym{CP}{CP}{Constraint Programming}
	\ouracronym{FP}{FP}{Functional Programming}
	\ouracronym{KR}{KR}{Knowledge Representation}
	\ouracronym{CSP}{CSP}{Constraint Satisfaction Problem}
	\ouracronym{SMT}{SMT}{SAT Modulo Theories}
	\ouracronym{KBS}{KBS}{Knowledge Base System}
	\ouracronym{NNF}{NNF}{Negation Normal Form}
	\ouracronym{FNNF}{FNNF}{Flat Negation Normal Form}
	\ouracronym{DefNNF}{DefNNF}{Definition Negation Normal Form}
	\ouracronym{DEFNF}{DEFNF}{Definition Normal Form}
	\newcommand{\DEFNNF}{\DefNNF} %Was previously called like this. Keeping consistency
	\ouracronym{CDCL}{CDCL}{Conflict-Driven Clause-Learning}
	\ouracronym{WFS}{WFS}{Well-Founded Semantics}
	\ouracronym{LCG}{LCG}{Lazy Clause Generation}
	\ouracronym{AEL}{AEL}{Autoepistemic Logic}
	\ouracronym{OEL}{OEL}{Ordered Epistemic Logic}
	\ouracronym{AFT}{AFT}{Approximation Fixpoint Theory}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%       DEFINITIONS: commands for writing definitions      %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Stuff for (delayed) definitions   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The only commands you should use explicitly are:
%	* Environment ldef for a logical definition (should be used in mathmode)
%	* Environment ltheo for a logical theory (starts mathmode itself)
%	* \LRule defines a rule, usage \LRule{HEAD}{BODY}{OPTIONAL: DELAY}{OPTIONAL: CONSTRUCTION}
% 		---> Can be used inside a ldef or an align environment
%% USAGE EXAMPLE:
% \begin{ltheo}
% \lnot S(1) \\
% \exists x\typed{D}: P(x) \\
% \forall x\typed{D}: P(x) \limpl R(x)\\
% \begin{ldef}
% \LRule{\forall x\typed{D}: R(x)}{ Q(x) \lor S(x)}{delay}{construction} \\
% \LRule{\forall x\typed{D}: R(x)}{ Q(x) \lor S(x)}{delay}{construction} \\
% \LRule{\forall x\typed{D}: R(x)}{ Q(x) \lor S(x)}{delay}{construction} \\
% \LRule{\forall x\typed{D}: Q(x)}{ R(x)}
% \end{ldef}
% \end{ltheo}
%
% You can use these rules in an align environment as follows:
% \begin{align*}
% \LRule{\forall x\typed{D}: R(x)}{ Q(x) \lor S(x)}{delay}{construction} \\
% \LRule{\forall x\typed{D}: R(x)}{ Q(x) \lor S(x)}{delay}{construction} \\
% \LRule{Q}{ R(x)}
% \end{align*}

	\makeatletter
	\def\ifenv#1{
	\def\@tempa{#1}%
	\def\@ttempa{#1*}%
	\ifx\@tempa\@currenvir
	\expandafter\@firstoftwo
	\else
	\expandafter\@secondoftwo
	\fi
	}
	\makeatother

%Delayed definition rule. Usage: \ddrule{HEAD}{BODY}{DELAY}{CONSTRUCTION}
	\newcommand{\ddrule}[4]{\ensuremath{#1 \leftarrow #2 & \{#3\} & #4}}
%Non-delayed definition rule. Usage: \drule{HEAD}{BODY}
	\newcommand{\drule}[2]{\ensuremath{#1 & \leftarrow & #2}}

%Delayed align rule. Usage: \darule{HEAD}{BODY}{DELAY}{CONSTRUCTION}
	\newcommand{\darule}[4]{\ensuremath{#1 \leftarrow #2 & \{#3\} & #4}}
%Non-delayed align rule. Usage: \arule{HEAD}{BODY}
	\newcommand{\arule}[2]{\ensuremath{#1 \, &\leftarrow \, #2}}

	\newenvironment{ldef}{\left\{\begin{array}{l@{ \,}l@{\,}l}}{\end{array}\right\}}
	\newenvironment{ltheo}{\[\begin{array}{l}}{\end{array}\]\ignorespacesafterend}

	\newcommand{\LNDRule}[2]{
	\ifenv{array}
	{\drule{#1}{#2}}
	{ \ifenv{align}
		{\arule{#1}{#2}}
		{\ifenv{align*}
		{\arule{#1}{#2}}
		{ERROR: using LDRule in unsupported environment: \@currenvir}
		}
	}
	}

	\newcommand{\LDRule}[4]{
	\ifenv{array}
	{\ddrule{#1}{#2}{#3}{#4}}
	{ \ifenv{align}
		{\darule{#1}{#2}{#3}{#4}}
		{\ifenv{align*}
		{\darule{#1}{#2}{#3}{#4}}
		{ERROR: using LDRule in unsupported environment: \@currenvir}
		}
	}
	}

% NOTE: if getting strange errors on alignments, you probably forgot the ldef environment
	\NewDocumentCommand\LRule{m+g+g+g}{%
		\IfNoValueTF{#2}%
		{#1.&}{%
		\IfNoValueTF{#3}
		{\LNDRule{#1}{#2.}}
		{\LDRule{#1}{#2.}{#3}{#4}}%
		}
	}



%FOR COMPLEX RULES: with a c above the lrule...

	\NewDocumentCommand\CLRule{m+g}{%
	\ifenv{array}
	{\cdrule{#1}{#2}}
	{ \ifenv{align}
		{\carule{#1}{#2}}
		{\ifenv{align*}
			{\carule{#1}{#2}}
			{ERROR: using CLRule in unsupported environment: \@currenvir}
		}
	}
	}

	\NewDocumentCommand\carule{m+g}{%
		\IfNoValueTF{#2}
			{\ensuremath{#1.}}
			{\ensuremath{#1 \, &\cause \, #2}}}
	\NewDocumentCommand\cdrule{m+g}{%
		\IfNoValueTF{#2}
			{\ensuremath{#1.}}
			{\ensuremath{#1 & \cause & #2}}}
	



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            Stuff for rules for state-changes in an algorithm             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The only commands you should use explicitly are:
%	* Environment lprop for a set of state-changing rules
%	* \AlgoRule defines a propagation rule, usage \AlgoRule{Name}{Previous state}{New state}{Condition}
% The whole environment is in MATH mode by default, so use hbox to obtain normal text.

	\newcommand{\algrule}[4]{
	\hbox{{#1}:}& 
	\quad #2 ~\longrightarrow~ #3 
	\hbox{~ if } #4\\
	}

	\newenvironment{lprop}{\[\begin{array}{ll}}{\end{array}\]}

	\newcommand{\AlgoRule}[4]{
	\ifenv{array}
	{\algrule{#1}{#2}{#3}{#4}}
		{ERROR: using AlgoRule in unsupported environment: \@currenvir}
	}


\newcommand{\commentstyle}{\color{Gray}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%                    In-paper commentstyle                     %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\newcommand{\ignore}[1]{}

%Boolean to quickly disable all comments
	\newboolean{nocomments}
	\setboolean{nocomments}{false}

%Boolean to decide whether we put our name in margin or not
	\newboolean{commentmargin}
	\setboolean{commentmargin}{true}

%General comments
	\newcommand{\namedcomment}[3]{%
		\ifthenelse{\boolean{nocomments}}%
		{}%IF no comments, write nothing
		{%Otherwise
			\ifthenelse{\boolean{commentmargin}}%
				{ {\color{#3} \marginpar{\color{#3}\sc #2}#1}  }%Name in margin
				{  {\color{#3} {\sc #2}: #1}  }%Name not in margin
		}%
	}
	\newcommand{\mnamedcomment}[3]{\ifthenelse{\boolean{nocomments}}{}{{\marginpar{ \color{#3}{\sc #2}:#1}}}}

	\newcommand{\namedchange}[4]{\marginpar{\color{#4}\sc #3}\textcolor{#4}{#1}\textcolor{gray}{\st{#2}}}

%todo's
	\newcommand{\todo}[1]{\namedcomment{#1}{TODO}{blue}}
	\newcommand{\todonm}[1]{{\color{blue}\sc TODO} #1}
	\newcommand{\mtodo}[1]{\mnamedcomment{#1}{TODO}{blue}}
	\newcommand{\old}[1]{\namedcomment{#1}{OLD}{gray}}

%Personal comments (KRR):
	\newcommand{\bart}[1]{\namedcomment{#1}{bb}{red}}
	\newcommand{\mbart}[1]{\mnamedcomment{#1}{bb}{red}}
	\newcommand{\gerda}[1]{\namedcomment{#1}{gj}{orange}}
	\newcommand{\marc}[1]{\namedcomment{#1}{md}{orange}}
	\newcommand{\joost}[1]{\namedcomment{#1}{jv}{purple}}
	\newcommand{\bdc}[1]{\namedcomment{#1}{bdc}{OliveGreen}}
	\newcommand{\broes}[1]{\namedcomment{#1}{bdc}{OliveGreen}}
	\newcommand{\mbroes}[1]{\mnamedcomment{#1}{bdc}{OliveGreen}}
	\newcommand{\pieter}[1]{\namedcomment{#1}{pvh}{NavyBlue}}
	\newcommand{\maurice}[1]{\namedcomment{#1}{mb}{orange}}
	\newcommand{\ingmar}[1]{\namedcomment{#1}{id}{purple}}
	\newcommand{\matthias}[1]{\namedcomment{#1}{mvdh}{blue}}
	\newcommand{\mmaurice}[1]{\mnamedcomment{#1}{mb}{orange}}
	\newcommand{\jo}[1]{ \namedcomment{#1}{jo}{Fuchsia}}
	\newcommand{\joachim}[1]{ \namedcomment{#1}{jj}{Sepia}}
	\newcommand{\mjoachim}[1]{ \mnamedcomment{#1}{jj}{Sepia}}
	\newcommand{\tim}[2]{\namedcomment{#1}{tvde}{brown}}
	\usepackage{soul}
	\newcommand{\bartch}[2]{\namedchange{#1}{#2}{bb}{red}}
	\newcommand{\broesch}[2]{\namedchange{#1}{#2}{bdc}{OliveGreen}}
%Personal comments  (Collaborations):
	\newcommand{\pjs}[1]{\namedcomment{#1}{pjs}{orange}}
	\newcommand{\jan}[1]{\namedcomment{#1}{jvdb}{orange}}
	\newcommand{\jvt}[1]{\namedcomment{#1}{jvt}{orange}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%                   Useful in-text commands                    %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newcommand{\keyword}[2]{%
% 	\expandafter\newcommand\csname #1\endcsname{#2\xspace}%
% 	\expandafter\newcommand\csname #1s\endcsname{#2s\xspace}%
% 	\expandafter\newcommand\csname #1ness\endcsname{#2ness\xspace}%
% % 	\expandafter\newcommand\MakeUppercase{\csname #1\endcsname}{#2\xspace}%
% %	\expandafter\newcommand\csname\makefirstuc{#1}\endcsname{\makefirstuc{#2}\xspace}%
% %	\expandafter\newcommand\csname\makefirstuc{#1}\endcsname{\makefirstuc{#2}s\xspace}%
% }


==> idp-latex/packages/xparse.tex <==
\usepackage{xparse}
